Revealing Decurve Flows for Generalized Graph Propagation

This study addresses the limitations of the traditional analysis of message-passing, central to graph learning, by defining {\em \textbf{generalized propagation}} with directed and weighted graphs. The significance manifest in two ways. \textbf{Firstly}, we propose {\em Generalized Propagation Neural Networks} (\textbf{GPNNs}), a framework that unifies most propagation-based graph neural networks. By generating directed-weighted propagation graphs with adjacency function and connectivity function, GPNNs offer enhanced insights into attention mechanisms across various graph models. We delve into the trade-offs within the design space with empirical experiments and emphasize the crucial role of the adjacency function for model expressivity via theoretical analysis. \textbf{Secondly}, we propose the {\em Continuous Unified Ricci Curvature} (\textbf{CURC}), an extension of celebrated {\em Ollivier-Ricci Curvature} for directed and weighted graphs. Theoretically, we demonstrate that CURC possesses continuity, scale invariance, and a lower bound connection with the Dirichlet isoperimetric constant validating bottleneck analysis for GPNNs. We include a preliminary exploration of learned propagation patterns in datasets, a first in the field. We observe an intriguing ``{\em \textbf{decurve flow}}'' - a curvature reduction during training for models with learnable propagation, revealing the evolution of propagation over time and a deeper connection to over-smoothing and bottleneck trade-off.

==> figures/curvature.tex <==
% \begin{tikzpicture}
% \node[inner sep=0pt] (g) at (0,0)
%     {\includegraphics[width=.20\textwidth]{iclr2023/figures/adj/g(0)_adj.pdf}};
% \node[inner sep=0pt] (g_cur) at (4,0)
%     {\includegraphics[width=.24\textwidth]{iclr2023/figures/curvature/g(0)_cur.pdf}};
% \node[inner sep=0pt] (whitehead) at (4, -3)
%     {\includegraphics[width=.22\textwidth]{iclr2023/figures/curvature/g(0)_hist_0.09324731677770615.pdf}};
% \draw[->,thick] (g) -- (g_cur)
%     node[fill=white] {};
% \node[inner sep=0pt] (g_cur) at (8,0)
%     {\includegraphics[width=.24\textwidth]{iclr2023/figures/curvature/Tir.pdf}};


    
% \end{tikzpicture}

==> others/exp_variants.tex <==



==> sections/preliminary.tex <==




